Efficient Large-Scale Domain Classification with Personalized Attention

In this paper, we explore the task of mapping spoken language utterances to one of thousands of natural language understanding domains in intelligent personal digital assistants (IPDAs). This scenario is observed for many mainstream IPDAs in industry that allow third parties to develop thousands of new domains to augment built-in ones to rapidly increase domain coverage and overall IPDA capabilities. We propose a scalable neural model architecture with a shared encoder, a novel attention mechanism that incorporates personalization information and domain-specific classifiers that solves the problem efficiently. Our architecture is designed to efficiently accommodate new domains that appear in-between full model retraining cycles with a rapid bootstrapping mechanism two orders of magnitude faster than retraining. We account for practical constraints in real-time production systems, and design to minimize memory footprint and runtime latency. We demonstrate that incorporating personalization results in significantly more accurate domain classification in the setting with thousands of overlapping domains.

==> excluded.tex <==
\section{Training Data Generation with Weak Supervision}
\label{sec:weak_supervision}
The presence of an extremely large number of mutually overlapping SLU domains means that eliciting large volumes of high quality human annotations to train our model is infeasible. Instead we adapt the weak supervision paradigm introduced by \cite{hoffmann2011knowledge}, which uses heuristic functions generate large numbers of noisy data samples. Clean data generation with weak supervision is a challenging problem, so we address it by decomposing it into two simpler problems.

\paragraph{Data Programming}

The key insight of the \textit{Data Programming} approach is that $O(1)$ simple labeling functions can be used to approximate $O(n)$ human annotated data points with much less effort. We adopt the formalism used by \cite{ratner2016data} to treat each of instance data generation rule as a rich generative model, defined by a labeling function $\lambda$ and describe different families of labeling functions. Our data programming pipeline is very simple and can be viewed analogous to the noisy channel model, first proposed for spelling correction by \cite{kernighan1990spelling} and used extensively for machine translation and speech recognition.
\begin{align*}
 \underset{\mu}{\argmax}\,P(\mu|s_i) = \underset{\mu}{\argmax} \,P(s_i|\mu).\,P(\mu)
\end{align*}
\noindent
where $\mu$ and $s_i$ represent utterances and the $i$th skill respectively. \DONE{DEFINE WHAT u, s and t ARE, THEN DEFINE WHAT THIS PROBABILITY DENOTES} $P(s_t|\mu)$ the probability of a skill being valid for an utterance is approximated by  simple functions that act as candidate data \textit{generators}  $\lambda_g \in \Lambda_g$ based on recognitions produced by a family of \textit{query patterns} $\lambda_q \in \Lambda_q$.  $P(\mu)$ is represented by a family of simple functions that act as \textit{noise detectors} $\lambda_n \in \Lambda_n$, which mark utterances as likely being noise.

We apply the technique to the query logs of a popular IPDA, which has support for personalized third party domains. Looking at the structure of utterances that match query pattern $\lambda_q$, each utterance of form \textit{"Ask \{Uber\} to \{get me a car\}"} can be considered as being parametrized by the underlying latent command $\mu_z$, that is \textit{"Get me a car"}, a target domain corresponding to service $s_t$, which in this case is \textit{Uber} and the query recognition pattern $\lambda_q$, in this case \textit{"Ask \{$s_t$\} to \{$\mu_z$\}"}. Next we assume that the distribution of latent commands over domains are independent of the query pattern.
\begin{align*}
P(\mu_z, s_t) \approx P(\mu, s_t, \lambda_q)
\end{align*}
Making this simple distributional approximation allows us to generate a large number of noisy training samples. The family of functions $\lambda_g \in \Lambda_g$ is thus defined such that $u_z = \lambda_g^i(\mu,\lambda_q^i)$

\DONE{WHAT IS SUBSCRIPT g OR q?, DEFINE IT}

\paragraph{Noise Reduction}
\label{ssec:data_filter}

% The distribution defined above contains a large number of noisy positive samples. Analogous to $P(\mu)$ in the noisy channel in the spell correction context, we have the function family $\Lambda_n$ to discard samples that are unlikely to be well formed.
% % \DONE{NOT CLEAR WHAT YOU MEAN HERE, WHAT NOISY CHANNEL IN WHAT CONTEXT?}
% % \DONE{YOU MAY WANT TO ENUMAREATE AS BULLETS EACH OF THE BELOW ITEMS BELOW TO IMPROVE CLARITY.}
% We defined a small family of heuristic noise detection functions $\lambda_n \in \Lambda_n$ based on domain specific features. For instance, 
% \begin{itemize}
%   \item $\lambda_n^1$ requires $u$ to contain a minimum threshold of information, thus as a rough heuristic we remove $\mu_z$ of token length less than 3. Utterances shorter than this mostly consist of non actionable commands.
%   \item  $\lambda_n^2$ \DONE{WHAT IS SUBSCRIPT n? THE NOTATION IS SLOPPY} applied a smoothing filter that discarded all data samples below a certain threshold of occurrences, utterances that are rarely observed are more likely to be ASR errors.
%   \item $\lambda_n^3$ places a constraint on the domains for which data is generated - if the domain is defined in such a way that it always produces the same semantic decoding irrespective of input, it cannot be trusted to generate valid data.
%   \item  $\lambda_n^4$ is a function that discards utterances that are classified as a built-in shared intent provided to the skill by the SDK. If multiple different skills re-use intents provided to them by the SDK, the data samples corresponding to intents be used to distinguish skills.
% \end{itemize}

The distribution defined above contains a large number of noisy positive samples. Related to $P(\mu)$ in the noisy channel in the spell correction context, we have the function family $\Lambda_n$ to discard samples that are unlikely to be well-formed.
% \DONE{NOT CLEAR WHAT YOU MEAN HERE, WHAT NOISY CHANNEL IN WHAT CONTEXT?}
% \DONE{YOU MAY WANT TO ENUMAREATE AS BULLETS EACH OF THE BELOW ITEMS BELOW TO IMPROVE CLARITY.}
We defined a small family of heuristic noise detection functions $\lambda_n \in \Lambda_n$ based on utterance-level and domain-level information. For instance,
\begin{itemize}
  \item $\lambda_n^1$ requires $u$ to contain a minimum threshold of information by removing those with $\mu_z$ that has token length fewer than 3. Utterances shorter than this mostly consist of non-actionable commands.
  \item  $\lambda_n^2$ \DONE{WHAT IS SUBSCRIPT n? THE NOTATION IS SLOPPY} discards all data samples below a certain threshold of occurrences, since utterances that are rarely observed are more likely to be ASR errors.
  \item $\lambda_n^3$ discards the data samples for a domain if they come from an overly broad pattern with a catch-all behavior.
  \item  $\lambda_n^4$ discards utterances that are classified as a built-in shared intent provided to the skills by the SDK. Such utterances are not domain-specific and cannot be said to belong to one specific domain.
\end{itemize}

% Each of these labeling functions $\lambda$ has a chance $\alpha$ of mislabeling an utterance, but we found this simple formulation works in practice.


\begin{figure}[!ht]
	\small
    \centering
    \includegraphics[width=0.7\columnwidth]{./fig/distribution_suggestion_final.pdf}
    \caption{\small Histogram of distribution of acceptance rate for utterance, domain pairs. X-axis denotes the accept rate and Y-axis denotes the portion of data.}
    \label{fig:histogram_accept_rate}
\end{figure}

\paragraph{Correlation with User Preference} To test the correlation of our system with observed user preferences, we use 2 months of data from a deployed system that recommends a third party domains in response to a user utterance, then gives the user the opportunity to either accept or reject the suggestion. Each data point consists of an utterance, a suggested domain and a binary indicator. The distribution (Figure \ref{fig:histogram_accept_rate}) is bimodal around 0 and 1. This data was binarized by discarding samples when we could not reject the hypothesis of true acceptance rate being greater than 0.4 for the negative samples, and vice versa for positive samples. This was done using a binomial test with 95\% confidence. Our model had a Pearson's correlation of 0.851 with the binary labels, as opposed to 0.312 for the baseline system. 
% These numbers are flawed because they only measure performance conditioned on the fact that the baseline system has already served the request to customers, which leads us to underestimate correlation scores due to biased sampling, but may hint that our model is better correlated with human judgment. 
\DONE {I CAN REALLY UNDERSTAND THE POINT OF THIS SECTION. NEEDS TO BE CLEAR, WHY THE CORRELATIONS ARE SO LOW?} 



